Chasing the Shadows: TTPs in Action to Attribute Advanced Persistent Threats

The current state of Advanced Persistent Threats (APT) attribution primarily relies on time-consuming manual processes. These include mapping incident artifacts onto threat attribution frameworks and employing expert reasoning to uncover the most likely responsible APT groups. This research aims to assist the threat analyst in the attribution process by presenting an attribution method named CAPTAIN (Comprehensive Advanced Persistent Threat AttrIbutioN). This novel APT attribution approach leverages the Tactics, Techniques, and Procedures (TTPs) employed by various APT groups in past attacks. CAPTAIN follows two significant development steps: baseline establishment and similarity measure for attack pattern matching. This method starts by maintaining a TTP database of APTs seen in past attacks as baseline behaviour of threat groups. The attribution process leverages the contextual information added by TTP sequences, which reflects the sequence of behaviours threat actors demonstrated during the attack on different kill-chain stages. Then, it compares the provided TTPs with established baseline to identify the most closely matching threat group. CAPTAIN introduces a novel similarity measure for APT group attack-pattern matching that calculates the similarity between TTP sequences. The proposed approach outperforms traditional similarity measures like Cosine, Euclidean, and Longest Common Subsequence (LCS) in performing attribution. Overall, CAPTAIN performs attribution with the precision of 61.36% (top-1) and 69.98% (top-2), surpassing the existing state-of-the-art attribution methods.

==> AttributionPerformance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{|cc|cccc|}
\hline
\multicolumn{2}{|c|}{}                                                                                                             & \multicolumn{4}{c|}{\textbf{Performance Metrics}}                                                                                                                                             \\ \cline{3-6} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{Method}}}                                                                                     & \multicolumn{1}{c|}{\textbf{Accuracy (\%)}}                    & \multicolumn{1}{c|}{\textbf{Precision (\%)}}                   & \multicolumn{1}{c|}{\textbf{Recall (\%)}}                      & \textbf{F1-score (\%)}                    \\ \hline
\multicolumn{1}{|c|}{}                                                                                                 & \textbf{Cosine}    & \multicolumn{1}{c|}{33.10}                        & \multicolumn{1}{c|}{58.17}                        & \multicolumn{1}{c|}{43.23}                        & 34.49                        \\ \cline{2-6} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Exp.-1:} Existence of \\ TTPs\end{tabular}}}            & \textbf{Euclidean} & \multicolumn{1}{c|}{40.0}                        & \multicolumn{1}{c|}{57.23}                        & \multicolumn{1}{c|}{53.65}                        & 38.73                        \\
\hline
\multicolumn{1}{|c|}{\textbf{Exp.-2:} TTPs Sequence}                                                                              & \textbf{LCS}       & \multicolumn{1}{c|}{33.10}                        & \multicolumn{1}{c|}{56.63}                        & \multicolumn{1}{c|}{44.25}                        & 34.30                        \\  \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Exp.-3:} Length and \\ Frequency patterns\end{tabular}}                  & \textbf{CAPTAIN}   & \multicolumn{1}{c|}{{\color[HTML]{212121} \textbf{55.17}}} & \multicolumn{1}{c|}{{\color[HTML]{212121} \textbf{61.36}}} & \multicolumn{1}{c|}{{\color[HTML]{212121} \textbf{64.74}}} & {\color[HTML]{212121} \textbf{52.72}} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Exp.-4:} Noor et al.  \\ \cite{Noor2019A}\end{tabular}} & \textbf{DLNN}      & \multicolumn{1}{c|}{46.21}                        & \multicolumn{1}{c|}{35.27}                        & \multicolumn{1}{c|}{36.67}                        & 34.37                        \\ \hline
\end{tabular}

==> RelatedWorkTTPXHunterComparison.tex <==
    \begin{tabular}
    {|p{4cm}|p{5cm}|p{1.3cm}|p{2cm}|p{2.5cm}|}
    % {|c|c|c|c|c|}
    \hline
    \textbf{Research work} & \textbf{Extraction technique} & \textbf{Sentence Context-aware} & \textbf{Identify relevant text} & \textbf{Range of MITRE ATT\&CK TTPs} \\
    \hline
    Legoy et al.~\cite{legoy2020automated} - rcATT & TF-IDF and ML Models (KNN, Decision Tree, Random Forest, and Extra Tree) & $\times$  & $\times$  & All TTPs\\
    \hline 
    Husari et al. \cite{Husari2017Ttpdrill}  & TF-IDF, Ontology-based, and improved BM25 similarity rank & $\times$ & $\checkmark$ & All TTPs\\
    \hline
    Li. et al. \cite{Li2022AttacKG} - AttacKG & Entity-based dependency graph and Graph-alignment algorithm & $\times$ & $\checkmark$ & All TTPs\\
    \hline
    Rani. et al \cite{Rani2023TTPHunter} - TTPHunter. & BERT/RoBERTa followed by Linear Classifier & $\checkmark$ & $\checkmark$ & 50 TTPs set Only\\
    \hline
    \textbf{TTPXHunter (Proposed)} & \textbf{Domain-specific SecureBERT with Linear Classifier} & $\checkmark$ & $\checkmark$ & \textbf{All TTPs}\\
    \hline
    \end{tabular}
